Facilities for Dark Energy Investigations

The discovery of cosmic acceleration has inspired ambitious experimental and observational efforts to understand its origin. Many of these take the form of large astronomical surveys, sometimes using new, special-purpose instrumentation, and in some cases entirely new facilities. This Report summarizes some of the major ongoing and planned dark energy experiments, focusing on those in which the U.S. community has a leading or significant supporting role. It provides background information for other Reports from the "Dark Energy and CMB" working group of the APS Division of Particles and Fields long-term planning exercise. We provide 1-2 page summaries of the SDSS-III Baryon Oscillation Spectroscopic Survey (BOSS) and its SDSS-IV successor eBOSS, the Dark Energy Survey (DES), the Subaru Hyper-Suprime Camera (HSC) and Prime Focus Spectrograph (PFS), the Hobby-Eberley Telescope Dark Energy Experiment (HEDTEX), the Dark Energy Spectroscopic Instrument (DESI), the Large Synpotic Survey Telescope (LSST), and the Euclid and AFTA-WFIRST (Wide Field Infrared Survey Telescope) space missions. Over the next one to two decades, these experiments seek to improve the precision of measurements of the cosmic expansion history and cosmic structure growth by factors of 10-100, while simultaneously increasing their redshift range and tightening control and cross-checks of sytematic effects. These measurements will dramatically improve the empirical constraints on theoretical explanations of cosmic acceleration and could lead to breakthroughs in our understanding of the nature of gravity and spacetime or the forms of energy present in the universe.

==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <16 Dec 93>.}
\typeout{NOTICE:  This macro file is NOT proprietary and may be 
freely copied and distributed.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt, 
%             for support of bold Greek
%
\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%

% The following was used for greek bf in the past.
% it is commented out for the time being
%
% Expands to hex digit corresponding to the value of the argument
%
%\def\hexnumber@#1{\ifnum#1<10 \number#1\else
% \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
% \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes. 
% Styles like Greekbf will hook in here.
%
%\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda 
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
%\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
%\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
%\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
%\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
%\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
%\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
%\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
%\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
%\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
%\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
%\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
%\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%




% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo} 
%
% lets you write 
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
% Newfields have a bad habit of putting blanks in front of
% and in back of their arguments.  Here are some macros to 
% remove the blanks

\def\eatfrontblank#1{#1}% TeX does this just by reading a parameter

\def\eatblank#1{\expandafter\eatfrontblank#1}
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%


